Searches for the rare hadronic decays $B^0 \rightarrow p\bar{p}p\bar{p}$ and $B^0_{s} \rightarrow p\bar{p}p\bar{p}$

Searches for the rare hadronic decays $B^0 \rightarrow p\bar{p}p\bar{p}$ and $B^0_{s} \rightarrow p\bar{p}p\bar{p}$ are performed using proton-proton collision data recorded by the LHCb experiment and corresponding to an integrated luminosity of 9$\rm{fb}^{-1}$. Significances of $9.3\,\sigma$ and $4.0\,\sigma$, including statistical and systematic uncertainties, are obtained for the $B^0 \rightarrow p\bar{p}p\bar{p}$ and $B^0_{s} \rightarrow p\bar{p}p\bar{p}$ signals, respectively. The branching fractions are measured relative to the topologically similar normalisation decays $B^0 \rightarrow J/\psi(\rightarrow p\bar{p}) K^{*0}(\rightarrow K^+ \pi^-)$ and $B^0_{s} \rightarrow J/\psi(\rightarrow p\bar{p}) \phi(\rightarrow K^+ K^-)$. The branching fractions are measured to be $ \mathcal{B}(B^0 \rightarrow p\bar{p}p\bar{p}) = ( 2.2 \pm 0.4 \pm 0.1 \pm 0.1 ) \times 10^{-8} $ and $ \mathcal{B}(B^0_{s} \rightarrow p\bar{p}p\bar{p}) = ( 2.3 \pm 1.0 \pm 0.2 \pm 0.1 ) \times 10^{-8}$. In these measurements, the first uncertainty is statistical, the second is systematic and the third one is due to the external branching fraction of the normalisation channel.

==> Makefile <==
# $Id: Makefile 87305 2016-02-08 13:50:32Z lafferty $
# ===============================================================================
# Purpose: simple Makefile to streamline processing latex document (just say "make" to execute)
# Author: Tomasz Skwarnicki
# Created on: 2010-09-24
# A few changes by Patrick Koppenburg on 2015-06-26
# ===============================================================================

# name of the main latex file (do not include .tex)
MAIN = main

# name of the target - change that to something descriptive, like paper-v0, Bs2PhiPhi-ANA-v1, etc...
TARGET = template

# name of command to perform Latex (either pdflatex or latex)
LATEX = pdflatex

ifeq ($(LATEX),pdflatex)
	FIGEXT = .pdf
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN)
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl
	BUILDCOMMANDUPRIGHT=rm -f upright.aux && $(LATEX) upright && bibtex upright && $(LATEX) upright && $(LATEX) upright
	MAKEMAINCOUNT= sed 's\#{wordcount}{false}\#{wordcount}{true}\#' main-prl.tex > main-count.tex
	BUILDCOMMANDCOUNT= $(MAKEMAINCOUNT) && rm -f $(MAIN)-count.aux && $(LATEX) $(MAIN)-count && bibtex $(MAIN)-count >/dev/null; true && $(LATEX) $(MAIN)-count && ./wordcount.sh $(MAIN)-count && rm wordcount.pdf main-count*
else
	FIGEXT = .eps
	MAINEXT= .pdf
	BUILDCOMMAND=rm -f $(MAIN).aux && $(LATEX) $(MAIN) && bibtex $(MAIN) && $(LATEX) $(MAIN) && $(LATEX) $(MAIN) && dvips -z -o $(MAIN).ps $(MAIN) && ps2pdf $(MAIN).ps && rm -f head.tmp body.tmp
	BUILDCOMMANDPRL=rm -f $(MAIN)-prl.aux && $(LATEX) $(MAIN)-prl && bibtex $(MAIN)-prl && $(LATEX) $(MAIN)-prl && $(LATEX) $(MAIN)-prl && dvips -z -o $(MAIN)-prl.ps $(MAIN)-prl && ps2pdf $(MAIN)-prl.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDUPRIGHT=rm -f upright.aux && $(LATEX) upright && bibtex upright && $(LATEX) upright && $(LATEX) upright && dvips -z -o upright.ps upright && ps2pdf upright.ps && rm -f head.tmp body.tmp
	BUILDCOMMANDCOUNT=
endif

# list of all source files
TEXSOURCES = $(wildcard *.tex) $(wildcard *.bib) $(wildcard *.bst)
FIGSOURCES = $(wildcard figs/*$(FIGEXT))
SOURCES    = $(TEXSOURCES) $(FIGSOURCES)

# define output (could be making .ps instead)
OUTPUT = $(TARGET)$(MAINEXT)

# cp temporary main.pdf to target.
$(OUTPUT): $(MAIN)$(MAINEXT)
	cp $(MAIN)$(MAINEXT) $(OUTPUT)

# prescription how to make output (your favorite commands to process latex)
# do latex twice to make sure that all cross-references are updated
$(MAIN)$(MAINEXT): $(SOURCES) Makefile
	$(BUILDCOMMAND)

# just so we can say "make all" without knowing the output name
all: $(OUTPUT)

# remove temporary files (good idea to say "make clean" before putting things back into repository)
.PHONY : clean
clean:
	rm -f *~ *.aux *.log *.bbl *.blg *.dvi *.tmp *.out *.blg *.bbl *.toc $(OUTPUT) $(MAIN)$(MAINEXT) $(MAIN).ps $(MAIN)-prl.ps $(MAIN)-prl.pdf

# remove output file
rmout:
	rm $(OUTPUT) $(MAIN)$(MAINEXT)

# Make the PRL version
prl:
	$(BUILDCOMMANDPRL)

# Make the PRL version
count:
	$(BUILDCOMMANDCOUNT)
	@echo ''
	@echo 'Figures:   Add 20+150/(aspect ratio) per figure'
	@echo 'Equations: Add 16 words per row (single column) '
	@echo 'Tables:    Add 13 words plus 6.5 words per line (single column)'
	@echo

# Make the upright version
upright:
	$(BUILDCOMMANDUPRIGHT)

